Learning Glioblastoma Tumor Heterogeneity Using Brain Inspired Topological Neural Networks

Accurate prognosis for Glioblastoma (GBM) using deep learning (DL) is hindered by extreme spatial and structural heterogeneity. Moreover, inconsistent MRI acquisition protocols across institutions hinder generalizability of models. Conventional transformer and DL pipelines often fail to capture the multi-scale morphological diversity such as fragmented necrotic cores, infiltrating margins, and disjoint enhancing components leading to scanner-specific artifacts and poor cross-site prognosis. We propose TopoGBM, a learning framework designed to capture heterogeneity-preserved, scanner-robust representations from multi-parametric 3D MRI. Central to our approach is a 3D convolutional autoencoder regularized by a topological regularization that preserves the complex, non-Euclidean invariants of the tumor's manifold within a compressed latent space. By enforcing these topological priors, TopoGBM explicitly models the high-variance structural signatures characteristic of aggressive GBM. Evaluated across heterogeneous cohorts (UPENN, UCSF, RHUH) and external validation on TCGA, TopoGBM achieves better performance (C-index 0.67 test, 0.58 validation), outperforming baselines that degrade under domain shift. Mechanistic interpretability analysis reveals that reconstruction residuals are highly localized to pathologically heterogeneous zones, with tumor-restricted and healthy tissue error significantly low (Test: 0.03, Validation: 0.09). Furthermore, occlusion-based attribution localizes approximately 50% of the prognostic signal to the tumor and the diverse peritumoral microenvironment advocating clinical reliability of the unsupervised learning method. Our findings demonstrate that incorporating topological priors enables the learning of morphology-faithful embeddings that capture tumor heterogeneity while maintaining cross-institutional robustness.

==> framework.tex <==
\begin{tikzpicture}[
  font=\small,
  node distance=10mm and 12mm,
  box/.style={draw, rounded corners, align=center, inner sep=6pt, text width=4.2cm},
  sbox/.style={draw, rounded corners, align=center, inner sep=6pt, text width=4.2cm, fill=gray!6},
  arrow/.style={-Latex, thick}
]

% -----------------------------
% DATA SOURCES
% -----------------------------
\node[box] (int) {Internal MRI cohorts\\UPENN + UCSF + RHUH\\4 modalities: T1,T1ce,T2,FLAIR};
\node[box, right=of int] (tcga) {External MRI cohort\\TCGA mapped to BraTS2021 folders\\4 modalities: T1,T1ce,T2,FLAIR};

% -----------------------------
% PREPROCESS
% -----------------------------
\node[sbox, below=of $(int)!0.5!(tcga)$] (prep) {Preprocessing per patient\\
Load 4 volumes $\rightarrow$ resample to $128^3$\\
Intensity normalization\\
Stack channels: $X \in \mathbb{R}^{4\times128\times128\times128}$};

\draw[arrow] (int) -- (prep);
\draw[arrow] (tcga) -- (prep);

% -----------------------------
% MODEL CORE
% -----------------------------
\node[box, below=of prep, text width=4.8cm] (enc) {3D Encoder CNN\\Conv3D + ReLU + Pool};
\node[box, right=of enc, text width=4.4cm] (emb) {Embedding layer\\Flatten + FC\\$z \in \mathbb{R}^{256}$};

\node[box, right=of emb, text width=4.4cm] (haz) {Survival branch\\hazard/logit $h$};
\node[box, below=of emb, text width=4.4cm] (dec) {Decoder\\FC + Deconv3D};
\node[box, below=of dec, text width=4.8cm] (recon) {Reconstruction output\\$\hat{X} \in \mathbb{R}^{4\times128\times128\times128}$};

\draw[arrow] (prep) -- (enc);
\draw[arrow] (enc) -- (emb);
\draw[arrow] (emb) -- (haz);
\draw[arrow] (emb) -- (dec);
\draw[arrow] (dec) -- (recon);

% Group box around model
\node[draw, rounded corners, inner sep=6pt, fit=(enc)(emb)(haz)(dec)(recon), label={[font=\small]above:TopoGBM Core Model (Encoder frozen at inference)}] (modelbox) {};

% -----------------------------
% OUTPUT ARTIFACTS
% -----------------------------
\node[sbox, left=of recon, text width=4.4cm] (outEmb) {Per-patient embeddings\\feat\_0..feat\_255\\(CSV artifacts)};
\node[sbox, right=of recon, text width=4.4cm] (outHaz) {Per-patient survival score\\hazard/risk (CSV artifacts)};

\draw[arrow] (emb) |- (outEmb);
\draw[arrow] (haz) |- (outHaz);

% -----------------------------
% RECON METRICS
% -----------------------------
\node[box, below=of recon, text width=5.2cm] (reconM) {Reconstruction metrics\\MAE, MSE, PSNR, SSIM\\+ MAE\_TUMOR / MAE\_NON\_TUMOR (if mask)};
\draw[arrow] (recon) -- (reconM);

\node[sbox, below left=of reconM, text width=4.6cm] (shift) {Internal vs TCGA shift\\Cohen's $d$, MWU $p$\\domain consistency};
\node[sbox, below right=of reconM, text width=4.6cm] (reconTbl) {Per-case tables\\internal\_recon\_metrics.csv\\tcga\_recon\_metrics.csv};

\draw[arrow] (reconM) -- (shift);
\draw[arrow] (reconM) -- (reconTbl);

% -----------------------------
% SURVIVAL EVAL
% -----------------------------
\node[box, below=of outHaz, text width=5.0cm] (survEval) {Survival evaluation (model-only)\\C-index (orientation checked)\\KM split with min-arm constraint\\ROC/AUC for 1y horizon (optional)};
\draw[arrow] (outHaz) -- (survEval);

% -----------------------------
% OPTIONAL SURVIVAL HEADS
% -----------------------------
\node[box, below=of outEmb, text width=5.0cm] (heads) {Optional downstream heads\\(train on internal embeddings)\\Penalized CoxPH / Discrete-time head\\Evaluate: internal test + TCGA};
\draw[arrow] (outEmb) -- (heads);

% -----------------------------
% REGION ATTRIBUTION
% -----------------------------
\node[box, below=of shift, text width=5.6cm] (attr) {Tumor-region attribution\\Mask source: UPENN seg or UCSF proxy\\Define regions: tumor + rings (0--20 vox)\\tissue non-tumor vs CSF-like\\Occlusion on GPU: $\Delta h$ and $\Delta z$\\Report: haz\_frac\_* and emb\_frac\_*};
\draw[arrow] (reconM) -- (attr);

% -----------------------------
% FINAL PAPER BUNDLE
% -----------------------------
\node[sbox, below=of $(heads)!0.5!(attr)$, text width=6.2cm] (paper) {Paper artifacts\\(Tables + Figures)\\Recon quality + domain shift\\Survival ranking/separation\\Tumor vs peri-tumor attribution summaries};

\draw[arrow] (survEval) |- (paper);
\draw[arrow] (heads) |- (paper);
\draw[arrow] (attr) -- (paper);

\end{tikzpicture}


==> methods.tex <==
\subsection{MRI Preprocessing and Topology-Aware Feature Embedding}

All T1-post contrast MRI volumes were preprocessed using a standard neuroimaging pipeline to reduce scanner- and acquisition-induced variability and to isolate tumor morphology:

\begin{enumerate}
    \item \textbf{Intensity non-uniformity correction} via N4 bias-field correction.
    \item \textbf{Cranial content extraction} using skull stripping.
    \item \textbf{Orientation normalization} to standard anatomical axes.
    \item \textbf{Resampling} to 1\,mm isotropic resolution.
    \item \textbf{Tumor-focused cropping}: 3D patches centered on the lesion were extracted using the union of enhancing tumor and necrotic core segmentation masks.
\end{enumerate}

These cropped volumes serve as inputs to a topology-aware CNN encoder that jointly learns appearance and shape. To expose the encoder to morphology, we compute differentiable topological summaries (persistent homology) from intermediate feature maps or segmentation probability fields, and regularize the learned embedding to preserve salient tumor topology (e.g., ring enhancement, necrotic cavities, infiltrative rims).

\subsubsection{Topological Representation Learning}

Let $\mathsf{D}^{(q)}_\mathrm{pred}$ and $\mathsf{D}^{(q)}_\mathrm{true}$ denote the predicted and reference persistence diagrams for homology dimension $q \in \{0,1,2\}$, computed from a cubical complex on a filtration (e.g., superlevel sets of a probability field or signed distance transform). For a topological feature $h_i$ with birth $b_i$ and death $d_i$, its \textbf{persistence} is:

\begin{equation}
p_i = d_i - b_i.
\label{eq:persistence}
\end{equation}



\begin{figure}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=8.5cm]{images/Testsurvival.png}}
%  \vspace{2.0cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{images/embeddings_tsne_by_Feature_201_test_UPENN.png}}
%  \vspace{1.5cm}
  \centerline{(b) Results 3}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{images/embeddings_tsne_by_Feature_252_test_RHUH.png}}
%  \vspace{1.5cm}
  \centerline{(c) Result 4}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
%
\end{figure}




We penalize discrepancies between predicted and true diagrams to ensure the encoder preserves creation/destruction of connected components ($H_0$), loops/rims ($H_1$), and voids/necrotic cavities ($H_2$). Two complementary losses are used:

\textbf{(A) Matched persistence MSE:}
\begin{equation}
\mathcal{L}_\mathrm{topo}^{(q)} = \sum_{i=1}^{N_q} \bigl(p_i^\mathrm{pred} - p_{\pi(i)}^\mathrm{true}\bigr)^2,
\label{eq:topo-mse}
\end{equation}
where $\pi$ is an optimal matching between features (e.g., Hungarian matching in Euclidean birth--death space), and $N_q$ is the number of matched features in dimension $q$.

\textbf{(B) Diagram distance (Wasserstein-2):}
\begin{equation}
\mathcal{W}_2\!\bigl(\mathsf{D}^{(q)}_\mathrm{pred}, \mathsf{D}^{(q)}_\mathrm{true}\bigr)
= \min_{\gamma \in \Gamma} \left( \sum_{(u,v)\in \gamma} \|u-v\|_2^2 \right)^{1/2},
\label{eq:wasserstein}
\end{equation}
where $\Gamma$ is the set of partial matchings augmented with diagonal projections. In practice, we use a differentiable relaxation so gradients flow to the encoder.

The overall topological regularizer aggregates across homology dimensions:
\begin{equation}
\mathcal{L}_\mathrm{topo} = \sum_{q \in \{0,1,2\}} \alpha_q \,\mathcal{L}_\mathrm{topo}^{(q)}.
\label{eq:topo-agg}
\end{equation}

\subsubsection{Full Encoder Objective}

The encoder is optimized using a composite loss that balances appearance fidelity, segmentation accuracy, and topological consistency:
\begin{equation}
\mathcal{L}_\mathrm{encoder}
= \lambda_\mathrm{rec}\,\mathcal{L}_\mathrm{rec}
+ \lambda_\mathrm{seg}\,\mathcal{L}_\mathrm{seg}
+ \lambda_\mathrm{topo}\,\mathcal{L}_\mathrm{topo}.
\label{eq:encoder-loss}
\end{equation}

Here, $\mathcal{L}_\mathrm{rec}$ is voxel-wise reconstruction error (e.g., mean squared error), and $\mathcal{L}_\mathrm{seg}$ is a compound segmentation loss (e.g., Dice + cross-entropy):
\begin{equation}
\mathcal{L}_\mathrm{rec} = \|x - \hat{x}\|_2^2,\qquad
\mathcal{L}_\mathrm{seg} = 1 - \mathrm{Dice}(y, \hat{y}) + \mathrm{CE}(y, \hat{y}).
\label{eq:rec-seg}
\end{equation}

The final patient-level \textbf{TopoEmbedding} is obtained via global average pooling of the deepest feature map, producing a $D=2048$-dimensional vector.

\subsection{Cross-Cohort Harmonization via PCA Scanner Bias Removal}

Because MRI acquisitions vary across institutions (e.g., manufacturer, field strength, coil geometry, pulse sequence), embeddings may encode scanner identity. To mitigate this, PCA is fit \textbf{only on the training cohorts} and bias directions are removed.

Given an embedding matrix $X \in \mathbb{R}^{N \times D}$ (rows: patients, columns: features), we compute:
\begin{equation}
Z = \mathrm{PCA}(X),
\label{eq:pca}
\end{equation}
and obtain the harmonized representation by discarding the first $k$ principal components (PCs) that capture scanner-specific variance:
\begin{equation}
\tilde{Z} = Z[:,\,k:D], \qquad k=3~\text{(typical)}.
\label{eq:pca-harmonized}
\end{equation}

\subsection{Transformer-Enhanced DeepSurv Architecture}

Each harmonized patient embedding $\tilde{z}_i \in \mathbb{R}^{d}$ is passed to a DeepSurv-style model augmented with \textbf{feature-attention gating}, \textbf{learnable tokenization}, and \textbf{Transformer encoders} to capture non-local interactions indicative of tumor topology and morphology.

\subsubsection{Feature-Attention Gating}

We compute a squeeze--excitation-like gate to emphasize informative coordinates:
\begin{equation}
g = \sigma\!\bigl(W_2\,\mathrm{ReLU}(W_1\,\tilde{z})\bigr),\qquad
\tilde{z}^{\ast} = g \odot \tilde{z},
\label{eq:gating}
\end{equation}
where $W_1 \in \mathbb{R}^{r \times d}$, $W_2 \in \mathbb{R}^{d \times r}$, $\sigma$ is the logistic sigmoid, and $\odot$ denotes elementwise multiplication.

\subsubsection{Learnable Tokenization}

To enable contextual modeling, the gated vector is linearly projected and reshaped into a sequence of latent tokens:
\begin{equation}
H = \mathrm{reshape}\!\bigl(W_p\,\tilde{z}^{\ast}\bigr) \in \mathbb{R}^{L \times d_\mathrm{model}},
\qquad
H' = H + P,
\label{eq:tokenization}
\end{equation}
where $P$ are learned positional encodings.

\subsubsection{Transformer Encoder for Morphological Interaction Modeling}

A 2-layer Transformer encoder models interactions across tokens. For multi-head self-attention (MHA) with $h$ heads:
\begin{equation}
\mathrm{MHA}(H') = \mathrm{concat}\bigl(A_1,\dots,A_h\bigr)W_O,
\label{eq:mha}
\end{equation}
\begin{equation}
A_m = \mathrm{softmax}\!\left(\frac{Q_m K_m^\top}{\sqrt{d_k}}\right)V_m,\quad
Q_m = H' W_Q^{(m)},\quad K_m = H' W_K^{(m)},\quad V_m = H' W_V^{(m)}.
\label{eq:attention-head}
\end{equation}

With residual and feed-forward blocks, the encoder output is:
\begin{equation}
\hat{H} = \mathrm{TransformerEncoder}(H'), \qquad
v = \frac{1}{L}\sum_{\ell=1}^{L} \hat{H}_\ell.
\label{eq:transformer-pool}
\end{equation}

\subsubsection{Survival Risk Estimation via Cox Proportional Hazards Head}

A fully connected MLP maps $v$ to a scalar log-risk:
\begin{equation}
\eta_i = \mathrm{MLP}(v_i).
\label{eq:log-risk}
\end{equation}

\subsection{Cox Partial Likelihood Optimization}

Let $T_i$ denote observed time, $\delta_i \in \{0,1\}$ the event indicator (1\,=\,death, 0\,=\,censored), and $\eta_i$ the predicted log-risk. Define the \textbf{risk set}:
\begin{equation}
\mathcal{R}_i = \{j \mid T_j \ge T_i\}.
\label{eq:risk-set}
\end{equation}

The negative Cox partial likelihood is:
\begin{equation}
\mathcal{L}(\theta) = - \sum_{i:\,\delta_i=1} \left(\eta_i - \log \sum_{j \in \mathcal{R}_i} e^{\eta_j}\right).
\label{eq:cox}
\end{equation}



% 3. WIDE STATISTICAL TABLE
\begin{table*}[!t]
\centering
\caption{Cross-cohort statistical comparison of reconstruction metrics and tumor signal enrichment.}
\label{tab:results_comparison}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l S[table-format=2.6] S[table-format=1.6] S[table-format=2.6] S[table-format=1.6] S[table-format=-1.6] S[table-format=1.2e-1]}
\toprule
& \multicolumn{2}{c}{\textbf{Internal cohort}} & \multicolumn{2}{c}{\textbf{TCGA cohort}} & & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Metric} & {\textbf{Mean}} & {\textbf{Std}} & {\textbf{Mean}} & {\textbf{Std}} & {\textbf{Cohen's $d$}} & {\textbf{MWU $p$-value}} \\
\midrule
MAE  & 0.038087 & 0.004488 & 0.037698 & 0.004619 & 0.085089  & 0.60 \\
MSE  & 0.009449 & 0.001563 & 0.009410 & 0.001800 & 0.022578  & 0.81 \\
PSNR & 20.504246 & 0.687816 & 20.533269 & 0.821030 & -0.037468 & 0.83 \\
SSIM & 0.658699 & 0.053129 & 0.695225 & 0.036057 & -0.846695 & 2.47e-07 \\
\bottomrule
\end{tabular}
\end{table*}





\subsection{External Validation}

\section{Methods: External Validation and Prognostic Generalizability}

\subsection{External Cohort Identification and Data Harmonization}
To evaluate the out-of-distribution generalizability of the \textit{JointTopoSurvivalNet}, we conducted an external validation using the TCGA-GBM (The Cancer Genome Atlas Glioblastoma Multiforme) cohort. Patient records were harmonized by mapping TCGA clinical identifiers to the BraTS2021 (Brain Tumor Segmentation) challenge identifiers via the TCIA Radiology Portal cross-reference. 

The primary endpoints were Overall Survival (OS), defined as the interval in days from diagnosis to death or last follow-up, and binary survival status. Let $T$ represent the time-to-event and $E$ represent the event indicator such that $E = 1$ if the event was observed and $E = 0$ if the data was right-censored.

\subsection{Volumetric Preprocessing Pipeline}
Input MRI volumes $\mathcal{V} \in \mathbb{R}^{H \times W \times D \times C}$ underwent a standardized preprocessing pipeline to ensure compatibility with the trained encoder:
\begin{itemize}
    \item \textbf{Intensity Normalization:} Voxel intensities were normalized via min-max scaling: 
    \begin{equation}
        \hat{v} = \frac{v - \min(v)}{\max(v) - \min(v) + \epsilon}
    \end{equation}
    \item \textbf{Isotropic Resampling:} To account for heterogeneous acquisition protocols, volumes were resampled to a fixed isotropic resolution of $128^3$ using trilinear interpolation.
    \item \textbf{Tensor Assembly:} Four core sequences (T1, T1Gd, T2, FLAIR) were concatenated to form a 4-channel input tensor.
\end{itemize}

\subsection{Deep Feature Extraction and Latent Space Analysis}
The pre-trained \textit{JointTopoSurvivalNet} was utilized as a static feature extractor. We focused on the bottleneck representation $\mathbf{z}$, which encapsulates both high-level semantic features and topological priors learned during the joint reconstruction and survival tasks. For each input volume $\mathbf{x}$, the 256-dimensional latent embedding was extracted from the penultimate layer:
\begin{equation}
    \mathbf{z} = \sigma(W_{fc} \cdot \phi_{enc}(\mathbf{x}) + b)
\end{equation}
where $\phi_{enc}$ represents the 3D convolutional backbone and $\sigma$ denotes the ReLU activation function.

\subsection{Statistical Evaluation and Survival Calibration}
Model performance was evaluated using Harrell’s Concordance Index ($C$-index) to measure the ability to rank patient risk:
\begin{equation}
    C = \frac{\sum_{i,j} \mathbb{1}_{T_i > T_j} \cdot \mathbb{1}_{\eta_i < \eta_j} \cdot E_j}{\sum_{i,j} \mathbb{1}_{T_i > T_j} \cdot E_j}
\end{equation}
where $\eta$ represents the predicted risk score from the downstream classifiers.

\subsection{Risk Stratification}
Patients were stratified into High-Risk and Low-Risk cohorts based on the median predicted hazard probability. Survival distributions were estimated using the Kaplan-Meier method:
\begin{equation}
    S(t) = \prod_{i: t_i \le t} \left( 1 - \frac{d_i}{n_i} \right)
\end{equation}
where $d_i$ is the number of events at time $t_i$ and $n_i$ is the number of subjects at risk.



==> methods3.tex <==
We present \textbf{TopoGBM} as a semi-supervised representational learning framework that (i) learns a compact multimodal latent space representation from 3D MRI via a reconstruction-driven encoder--decoder, (ii) uses the learned embedding (optionally fused with clinical covariates such as age) for survival risk prediction iii) represents the learnt embeddings from tumor and non-tumor regions for clinical relevance instead of being a black box. 
For training TopoGBM we used 3 multicenter cohorts : the University of Pennsylvania Glioblastoma (UPenn) dataset (n=627) \cite{bakas2022university}, the University of California San Francisco Preoperative Diffuse Glioma MRI (UCSF) dataset (n=398) \cite{calabrese2022university} and the Rio Hortega University Hospital Glioblastoma (RHUH) dataset (n=34) \cite{cepeda2023rio}. We split the datasets into a training set (UPENN=492, UCSF=321, RHUH=24) and unseen testing set (UPENN=135, UCSF=77, RHUH=10). For external unseen validation we use the Cancer Genome Atlas glioblastoma cohort (n=97) \cite{bakas2017advancing,bakas2017segmentation, menze2014multimodal}.
Let $i\in\{1,\dots,N\}$ index patients. 
Each patient has four co-registered MRI modalities :
\begin{equation}
X_i = \big[X_i^{(\mathrm{T1})},\,X_i^{(\mathrm{T1ce})},\,X_i^{(\mathrm{T2})},\,X_i^{(\mathrm{FLAIR})}\big].
\end{equation}
Survival outcomes are given by observed time and censoring indicator ($t_i \in \mathbb{R}_{>0}$,$e_i\in\{0,1\}$):
where $e_i=1$ indicates an event (e.g., death) and $e_i=0$ indicates right-censoring.
Optionally, a clinical covariate vector is provided ($a_i \in \mathbb{R}^{p}$). $p=1$in our age-only attention-head implementation.
$\Omega$ the voxel lattice defined as $\Omega=\{1,\dots,D\}\times\{1,\dots,H\}\times\{1,\dots,W\}$.
%\subsection{Input Pre-processing and Tensor Construction}
%\label{sec:preprocess}
TopoGBM processes standardized 3D volumes of fixed spatial size. Each NIfTI volume is resampled (via trilinear interpolation) to a common grid size $(D,H,W)$ (\ $128\times128\times128$, raw voxel intensity  $x\in\mathbb{R}$). For each modality volume, we apply intensity min-ax normalization \cite{sinsomboonthong2022performance}.
%where $x_{\min}$ and $x_{\max}$ are the minimum and maximum voxel intensities within that 3D modality volume (per patient).
The resulting input tensor is $\tilde{X}_i \in [0,1]^{4\times D\times H\times W}$.
\subsection{Stage 1: Joint Representation Learning}
\label{sec:stage1}
Here an encoder $f_{\theta}$ is trained to map multimodal MRI volumes to a latent embedding, and a decoder $g_{\phi}$ that reconstructs the input (embedding dimension $d=256$).
\begin{equation}
z_i = f_{\theta}(\tilde{X}_i) \in \mathbb{R}^{d},
\qquad
\hat{X}_i = g_{\phi}(z_i) \in \mathbb{R}^{4\times D\times H\times W},
\end{equation}
%\subsubsection{3D Convolutional Encoder}
%\label{sec:encoder}
The encoder is a sequence of 3D convolution blocks. For layer $\ell$, let $h_i^{(\ell)}$ be the feature map. A block is represented by:
\begin{equation}
u_i^{(\ell)} = \mathrm{Conv3D}\!\left(h_i^{(\ell-1)};W^{(\ell)},b^{(\ell)}\right),
\end{equation}
\begin{equation}
v_i^{(\ell)} = \sigma\!\left(u_i^{(\ell)}\right),
\end{equation}
\begin{equation}
h_i^{(\ell)} = \mathrm{Pool3D}\!\left(v_i^{(\ell)}\right),
\end{equation}
where $\sigma(\cdot)$ is a pointwise nonlinearity (ReLU \cite{agarap2018deep}) and $\mathrm{Pool3D}$ is max-pooling with stride 2.
After $L$ blocks, the output feature map is flattened, given by $\mathrm{flat}_i = \mathrm{Flatten}\!\left(h_i^{(L)}\right)$:
and projected to the latent space by a linear layer $z_i = W_z\,\mathrm{flat}_i + b_z.$
%\subsubsection{3D Decoder and Reconstruction}
%\label{sec:decoder}
The decoder expands the embedding back to a flattened feature tensor, reshaping, and applying transposed 3D convolutions:
\begin{equation}
\mathrm{flat}'_i = W_d z_i + b_d,
\qquad
H_i^{(0)} = \mathrm{Reshape}(\mathrm{flat}'_i),
\end{equation}
followed by upsampling blocks (ConvTranspose3D, \cite{paszke2019pytorch}):
\begin{equation}
H_i^{(m+1)} = \sigma\!\left(\mathrm{ConvTrans3D}(H_i^{(m)})\right),
\end{equation}
ending in a 4-channel reconstruction $\hat{X}_i$.
\begin{figure}[!ht]
  \centering
  \captionsetup{font=footnotesize}
  \includegraphics[width=0.8\columnwidth,
    trim={3pt 3pt 2.5pt 2.5pt},clip]{images/regional_attribution.pdf}
  \caption{The regional attribution for top-performing exemplars in the expert-verified UPENN and TCGA cohorts, revealing a high degree of spatial alignment between Hazard Fractions (solid, left bars) and Embedding Fractions (hatched, right bars). Nearly 50\% of the model's sensitivity is concentrated within the tumor and immediate peri-tumoral rings (0–20 voxels), demonstrating that the prognostic survival signal is intrinsically anchored to the topologically-encoded tumor morphology rather than healthy anatomical variance.}
  \label{fig:regional_attrib}
  \vspace{-14pt}
\end{figure}
%\subsubsection{Stage 1 Objective}
%\label{sec:reconloss}
The objective is to minimize voxel reconstruction error using mean-squared error (MSE) across channels and voxels:
\begin{equation}
\mathcal{L}_{\mathrm{recon}}(\theta,\phi)
=
\frac{1}{N}\sum_{i=1}^{N}
\frac{1}{4|\Omega|}
\sum_{c=1}^{4}\sum_{v\in\Omega}
\left(\tilde{X}_i^{(c)}(v) - \hat{X}_i^{(c)}(v)\right)^2.
\end{equation}
%(We also report MAE, PSNR, SSIM as evaluation metrics in Sec.~\ref{sec:reconmetrics}.)

\subsection{Stage 2: Survival Prediction using Attention}
\label{sec:stage2}
We predict discrete-time survival risk using the learned embedding $z_i$ and a clinical covariate vector $a_i$ (age).
%This is exactly where age is used:
%\begin{itemize}
%\item $a_i$ is batch-normalized (clinical normalization),
%\item projected to an attention query vector,
%\item used as the \emph{query} in multi-head attention over embedding-derived key/value vectors,
%\item and the fused representation is used to output survival-bin logits.
%\end{itemize}

%\subsubsection{Clinical Input and Where Age Enters the Model}
%\label{sec:agewhere}
Let $a_i\in\mathbb{R}^{p}$ be clinical covariates (here $p=1$ for age).
The attention head receives \emph{two} inputs $x^{\mathrm{feat}}_i := z_i \in \mathbb{R}^{d},
\qquad
x^{\mathrm{clin}}_i := a_i \in \mathbb{R}^{p}.$:
Thus, age is explicitly used as $x^{\mathrm{clin}}_i$.
%\subsubsection{Feature Filtering (Gating) on Embedding}
%\label{sec:gating}
Before fusion, a learned feature filter applies a multiplicative gate to the embedding:
\begin{equation}
g_i = \sigma\!\left(W_2\,\sigma(W_1 x^{\mathrm{feat}}_i + b_1) + b_2\right)\in(0,1)^d,
\end{equation}
where $\odot$ is elementwise multiplication, $\tilde{x}^{\mathrm{feat}}_i = x^{\mathrm{feat}}_i \odot g_i,$ and $\sigma(\cdot)$ is the sigmoid.
%This enforces a learned ``soft selection'' of embedding dimensions.%\subsubsection{Clinical Normalization and Projection}
%\label{sec:clinproj}
Clinical variables are batch-normalized and both feature and clinical vectors are projected to a common attention space of dimension $m$:
%\begin{equation}
%\tilde{x}^{\mathrm{clin}}_i = \mathrm{BN}(x^{\mathrm{clin}}_i),
%\end{equation}
\begin{equation}
f_i = \mathrm{LN}(W_f \tilde{x}^{\mathrm{feat}}_i + b_f)\in\mathbb{R}^{m},
\end{equation}
\begin{equation}
c_i = \mathrm{LN}(W_c \tilde{x}^{\mathrm{clin}}_i + b_c)\in\mathbb{R}^{m},
\end{equation}
where $\mathrm{LN}$ denotes layer normalization.
To interface with the Multi-head Attention formulation, we treat each modality as a single-token sequence by transposing the projected vectors:
%\begin{equation}
%F_i = f_i^\top \in \mathbb{R}^{1\times m},
%\qquad
%C_i = c_i^\top \in \mathbb{R}^{1\times m}.
%\end{equation}
%\begin{equation} F_i = f_i^\top \in \mathbb{R}^{1 \times m}, \quad C_i = c_i^\top \in \mathbb{R}^{1 \times m}. 
%\end{equation}
%\subsubsection{Multi-Head Attention with Clinical Query}
%\label{sec:attn}
Multi-head attention fuses clinical and imaging embedding information:
\begin{equation}
\mathrm{Attn}(Q,K,V)=\mathrm{softmax}\!\left(\frac{QK^\top}{\sqrt{m}}\right)V.
\end{equation}
In the implemented head, clinical is the query, and embedding features are key/value ($Q_i=C_i, K_i=F_i, V_i=F_i.$)With multi-head attention, $Q,K,V$ are linearly projected per head, attention is computed per head, and then concatenated and projected back to $\mathbb{R}^{m}$. Denoting the attention output by $A_i\in\mathbb{R}^{1\times m}$:
\begin{equation}
A_i = \mathrm{MHA}(Q_i,K_i,V_i).
\end{equation}
A residual ``clinical-centric fusion'' is used ($U_i = C_i + A_i.$)
Finally, $U_i$ is squeezed to a vector $u_i\in\mathbb{R}^{m}$.
%\subsubsection{Discrete-Time Survival Logits}
%\label{sec:discretelogits}
The fused vector is mapped to logits over $K$ discrete survival bins ($K=5$):
\begin{equation}
\ell_i = \mathrm{MLP}(u_i)\in\mathbb{R}^{K}.
\end{equation}
%In code, the MLP uses SELU + AlphaDropout:
%\begin{equation}
%\ell_i
%=%W_o\,\mathrm{AlphaDrop}\Big(\mathrm{SELU}(W_h u_i + b_h)\Big)+b_o.
%\end{equation}
%\subsection{Discrete-Time Label Construction and Loss}
%\label{sec:discreteloss}
We convert continuous survival time into a discrete bin label $y_i\in\{0,1,\dots,K-1\}$. Let the bin edges be
\begin{equation}
0=\tau_0 < \tau_1 < \cdots < \tau_{K-1} < \tau_K=\infty.
\end{equation}
A standard construction is $y_i = \max\{k:\tau_k \le t_i\}$.
%optionally with event-aware binning (e.g.\ quantiles of event times) and an analysis horizon (e.g.\ $t_i$ truncated at $H$ days).
With logits $\ell_i\in\mathbb{R}^{K}$ and class label $y_i$:
\begin{equation}
p_i(k)=\frac{\exp(\ell_i(k))}{\sum_{j=0}^{K-1}\exp(\ell_i(j))},
\qquad
\mathcal{L}_{\mathrm{CE}} = -\frac{1}{N}\sum_{i=1}^{N}\log p_i\!\left(y_i\right).
\end{equation}
%\subsection{Continuous Risk Score from Discrete Logits}
%\label{sec:risk}
To evaluate concordance, logits are converted to a continuous risk score. The expected bin index is $\mathbb{E}[b_i] = \sum_{k=0}^{K-1} k\,p_i(k)$:
In our implementation, earlier bins correspond to earlier death; therefore, higher hazard should correspond to smaller $\mathbb{E}[b_i]$. We define risk as the negated expected bin:
\begin{equation}
r_i = -\mathbb{E}[b_i] = -\sum_{k=0}^{K-1} k\,p_i(k).
\end{equation}
The survival attention head is trained with AdamW($\eta = 5\times10^{-5}$,$\lambda=5\times10^{-2}$):
%\begin{equation}
%\theta \leftarrow \theta - \eta\left(\nabla_{\theta}\mathcal{L} + \lambda\,\theta\right),
%\end{equation}
where $\eta$ is the learning rate and $\lambda$ is weight decay.
%We use:
%\begin{equation}
%\eta = 5\times10^{-5},\quad \lambda=5\times10^{-2},
%\end{equation}
\text{Here epochs}$=100$,\quad \text{patience}$=15$.
At each epoch, we compute validation concordance $C_{\mathrm{val}}$ and retain the model with best $C_{\mathrm{val}}$ (early stopping when no improvement beyond a tolerance for 'patience' epochs incorporated).
\textbf{Evaluation Metrics: }
For predicted risk scores $r_i$, concordance index is given by:
\begin{equation}
\mathrm{C}\text{-}\mathrm{index}
=
\Pr\left(r_i > r_j \;\middle|\; t_i < t_j,\; e_i=1\right),
\end{equation}
For each evaluated cohort the trained model outputs:
\begin{equation}
r_i,\quad
\hat{y}_i=\arg\max_k p_i(k),\quad
p_i(0),\dots,p_i(K-1).
\end{equation}
\begin{figure}[!ht]
  \centering
  \captionsetup{font=footnotesize}
  \includegraphics[width=.80\columnwidth,
    trim={5pt 4pt 5pt 4pt},clip]{images/reconupenntcga.pdf}
  \caption{Representative examples from internal UPENN (top 3 rows) and external TCGA/BraTS (bottom 3 rows) showing ground-truth FLAIR with expert tumor mask, reconstructed FLAIR, and the absolute reconstruction error  over the 4 modalities). Across cohorts, the autoencoder preserves global anatomy while residual error concentrates in and around tumor regions, visually supporting tumor-enriched reconstruction discrepancies under domain shift.}
  \label{fig:recon_figure}
\end{figure}
% ============================================================
% Additional TopoGBM components (recommended if included in paper)
% ============================================================
%\subsection{Reconstruction Metrics (Internal and External)}
%\label{sec:reconmetrics}
We quantify reconstruction fidelity with mean absolute error (MAE), mean squared error (MSE), peak signal-to-noise ratio (PSNR), and structural similarity (SSIM).
For a modality channel $c$:
\begin{equation}
\mathrm{MAE}^{(c)}_i=\frac{1}{|\Omega|}\sum_{v\in\Omega}\left|X^{(c)}_i(v)-\hat{X}^{(c)}_i(v)\right|,
\end{equation}
\begin{equation}
\mathrm{MSE}^{(c)}_i=\frac{1}{|\Omega|}\sum_{v\in\Omega}\left(X^{(c)}_i(v)-\hat{X}^{(c)}_i(v)\right)^2.
\end{equation}
Overall metrics are averaged across modalities.
%\begin{equation}
%\mathrm{MAE}_i=\frac{1}{4}\sum_{c=1}^{4}\mathrm{MAE}^{(c)}_i,
%\end{equation}
%\begin{equation}
%\mathrm{MSE}_i=\frac{1}{4}\sum_{c=1}^{4}\mathrm{MSE}^{(c)}_i.
%\end{equation}
With intensity range normalized to $[0,1]$. SSIM is computed on a subset of axial slices:$\mathrm{SSIM}_i = \frac{1}{|\mathcal{Z}|}\sum_{z\in\mathcal{Z}} \mathrm{SSIM}\!\left(X_i(\cdot,z),\,\hat{X}_i(\cdot,z)\right)$, $\mathrm{PSNR}_i = 10\log_{10}\left(\frac{1}{\mathrm{MSE}_i+\epsilon}\right)$
where $\mathcal{Z}$ are slices sampled between 20\% and 80\% of the depth to avoid extreme boundary slices.
%\subsection{Tumor vs Non-Tumor Reconstruction Error}
%\label{sec:tumornontumor}
Given a tumor mask $M_i\subset\Omega$, we compute region-restricted MAE:
\begin{equation}
\mathrm{MAE}_{i,\mathrm{tissue}}^{(c)}
=
\frac{1}{|M_i|}
\sum_{v\in M_i}
\left|X_i^{(c)}(v)-\hat{X}_i^{(c)}(v)\right|,
\end{equation}
%\begin{equation}
%\mathrm{MAE}_{i,\mathrm{non}}^{(c)}
%=
%\frac{1}{|\Omega\setminus M_i|}
%\sum_{v\notin M_i}
%\left|X_i^{(c)}(v)-\hat{X}_i^{(c)}(v)\right|.
%\end{equation}
Aggregating across modalities:
\begin{equation}
\mathrm{MAE}_{i,\mathrm{tissue}}=\frac{1}{4}\sum_{c=1}^{4}\mathrm{MAE}_{i,\mathrm{tissue}}^{(c)},
\end{equation}
%\begin{equation}
%\mathrm{MAE}_{i,\mathrm{non}}=\frac{1}{4}\sum_{c=1}^{4}\mathrm{MAE}_{i,\mathrm{non}}^{(c)}.
%\end{equation}
Here $tissue$ implies for tumor and non-tumor region separately. Our software implementation of TopoGBM will be released on GitHub upon acceptance of the manuscript.
%\subsection{Statistical Comparisons Across Cohorts}
%\label{sec:stats}
%To compare reconstruction metrics across cohorts we use Mann--Whitney U test \cite{mcknight2010mann} for distributional differences and Cohen's $d$ \cite{diener2010cohen} for effect size:
%\begin{equation}
%d = \frac{\mu_1-\mu_2}{s_p},
%\qquad
%s_p=\sqrt{\frac{(n_1-1)s_1^2+(n_2-1)s_2^2}{n_1+n_2-2}}.
%\end{equation}
%We quantify monotonic association between tumor fraction and tumor-region error using Spearman correlation \cite{myers2004spearman}
%\begin{equation}
%\rho_s = \mathrm{corr}\big(\mathrm{rank}(\mathrm{tumor\_frac}_i),\;\mathrm{rank}(\mathrm{MAE}_{i,\mathrm{tum}})\big).
%\end{equation}


==> results2.tex <==


\begin{center}
\captionof{table}{Comparison of Model Performance (C-index) and Explainability}
\label{tab:resultscindexexp}
\small % Reduces font size to small
\setlength{\tabcolsep}{2pt} % Tightens columns to save space
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{Test} & \textbf{External} & \textbf{Explainable} \\
                & (UPENN+UCSF+RHUH) & (TCGA) & \\
\hline
DeepSurv\cite{cerono2024clinical}& 0.64 & 0.48 & x \\
Transformer\cite{gomaa2024comprehensive} & 0.36 & 0.51 & x \\
SurvNet\cite{lyu2024survnet} & 0.47 & 0.57 & x \\
\textbf{TopoGBM (Ours)} & \textbf{0.67} & \textbf{0.58} & \checkmark \\
\hline
\end{tabular}
\end{center}


% 1. PERFORMANCE TABLE
\begin{table}[!htbp]
\centering
\caption{Comparison of Model Performance (C-index) and Explainability}
\label{tab:resultscindexexp}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Test} & \textbf{External} & \textbf{Explainable} \\
 & (Internal) & (TCGA) & \\
\midrule
DeepSurv \cite{cerono2024clinical} & 0.64 & 0.48 & $\times$ \\
Transformer \cite{gomaa2024comprehensive} & 0.36 & 0.51 & $\times$ \\
SurvNet \cite{lyu2024survnet} & 0.47 & 0.57 & $\times$ \\
\textbf{TopoGBM (Ours)} & \textbf{0.67} & \textbf{0.58} & \checkmark \\
\bottomrule
\end{tabular}
\end{table}

TopoGBM achieves a state-of-the-art C-index of 0.67 on the internal test set and 0.58 on the external TCGA cohort. Existing baselines show significant degradation, often falling to near-random levels.

% 2. RECONSTRUCTION STRATIFIED TABLE
\begin{table}[!htbp]
\centering
\caption{Reconstruction performance stratified by tumor vs non-tumor regions.}
\label{tab:recon_summary}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l l c c}
\toprule
\textbf{Dataset} & \textbf{Metric} & \textbf{Mean} & \textbf{Std} \\
\midrule
Internal & MAE (overall)  & 0.0381 & 0.0045 \\
Internal & MAE\textsubscript{tumor} & 0.1807 & 0.0266  \\
Internal & MAE\textsubscript{non-tumor} & 0.0381 & 0.0048  \\
\midrule
TCGA & MAE (overall) & 0.0377 & 0.0046 \\
TCGA & MAE\textsubscript{tumor} & 0.1898 & 0.0329  \\
TCGA & MAE\textsubscript{non-tumor} & 0.0359 & 0.0047 \\
\bottomrule
\end{tabular}
\end{table}

% 3. WIDE STATISTICAL TABLE
\begin{table*}[!t]
\centering
\caption{Cross-cohort statistical comparison of reconstruction metrics and tumor signal enrichment.}
\label{tab:results_comparison}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l S[table-format=2.6] S[table-format=1.6] S[table-format=2.6] S[table-format=1.6] S[table-format=-1.6] S[table-format=1.2e-1]}
\toprule
& \multicolumn{2}{c}{\textbf{Internal cohort}} & \multicolumn{2}{c}{\textbf{TCGA cohort}} & & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Metric} & {\textbf{Mean}} & {\textbf{Std}} & {\textbf{Mean}} & {\textbf{Std}} & {\textbf{Cohen's $d$}} & {\textbf{MWU $p$-value}} \\
\midrule
MAE  & 0.038087 & 0.004488 & 0.037698 & 0.004619 & 0.085089  & 0.60 \\
MSE  & 0.009449 & 0.001563 & 0.009410 & 0.001800 & 0.022578  & 0.81 \\
PSNR & 20.504246 & 0.687816 & 20.533269 & 0.821030 & -0.037468 & 0.83 \\
SSIM & 0.658699 & 0.053129 & 0.695225 & 0.036057 & -0.846695 & 2.47e-07 \\
\bottomrule
\end{tabular}
\end{table*}

% 4. SPEARMAN TABLE
\begin{table}[!htbp]
\centering
\caption{Spearman Rank Correlation between Tumor Fraction and Reconstruction Metrics.}
\label{tab:spearman_results}
\small
\begin{tabular}{llccS[table-format=-1.4]S[table-format=1.6]}
\toprule
\textbf{Dataset} & \textbf{Metric (y)} & \textbf{N} & \textbf{$r_s$} & \textbf{$p$-value} \\
\midrule
Internal & $\text{MAE}_{\text{Tumor}}$ & 28 & -0.2649 & 0.1731 \\
TCGA     & $\text{MAE}_{\text{Tumor}}$ & 97 & -0.3525 & 0.0004 \\
\midrule
Internal & Ratio ($\rho$) & 28 & -0.2315 & 0.2358 \\
TCGA     & Ratio ($\rho$) & 97 & -0.1601 & 0.1174 \\
\bottomrule
\end{tabular}
\end{table}

%\clearpage % THIS FORCES THE TABLES TO RENDER BEFORE THE NEXT SECTION
